Is two greater than one?: Analyzing Multipath TCP over Dual-LTE in the Wild

Multipath TCP (MPTCP) is a standardized TCP extension which allows end-hosts to simultaneously exploit all of their network interfaces. The recent proliferation of dual-SIM mobile phones makes multi-LTE MPTCP setup an attractive option. We perform extensive measurements of MPTCP over two LTE connections in low and high-speed mobility scenarios over five months, both in controlled and in-the-wild environments. Our findings indicate that MPTCP performance decreases at high speeds due to increased frequency of signal strength drops and handovers. Both LTE paths experience frequent changes which result in a sub-optimal subflow utilization. We also find that while path changes are unpredictable, their impact on MPTCP follows a deterministic trend. Finally, we show that both application traffic patterns and congestion control variants impact MPTCP adaptability at high speeds.

==> controlledExperiments.tex <==
%\section{Controlled Measurements} \label{sec:controlled}
%
%We first study MPTCP performance over multiple LTE connections in a controlled experiment setup. 
%%
%%This gives us insight into workings of MPTCP and its performance during access network vagaries due to handovers and signal drops.
%This allows us to analyze inner workings of MPTCP in the midst of access network vagaries in different moving speeds.

%\subsection{Experiment Setup}

%We set our mobile client to periodically download a 300~MB file\footnote{We do not use a smaller file in our tests as MPTCP is known to perform poorly for small object downloads~\cite{chen2013imc}.} from a remote server in three different mobility scenarios.
%
%We consciously did not consider a smaller file in our setup as it has been established in past studies that MPTCP does not perform well for small file download/upload due to slow start phase of each individual TCP subflow [cite].
% 
%We detail our mobility scenarios below:

%\begin{enumerate}[wide, labelwidth=!, labelindent=0pt]
%\item \textit{Stationary:} We ran multiple tests in different locations in Helsinki city center where client was stationary throughout transfer. Both LTE connections reported high signal strength. 
%\item \textit{Walking:} We walk a circular route of 4~km circumference around city center multiple times. Both ISPs have heavy LTE base station deployment along the route. 
%%
%%We conducted the experiments during late nights on weekdays such that our connectivity is minimally impaired by pre-existing loading of associated base stations by competing traffic.
%%
%The average walking speed reported at the end of the test was $\approx8$~km/h. 
%
%
%\item \textit{Driving:} We ran several tests while driving on a 13~km long inter-city highway at an average speed of 100~km/h without any intermediate stops.
%%
%The base station density of both ISPs alongside the route is shown in Figure~\ref{fig:driveHeatmap}.
%%
%%The central cluster for each ISP in the figure maps to around 30 base stations.
%% 
%During the test, we placed the RPi near the windshield to avoid any signal shielding by chassis of the vehicle.
%\end{enumerate}

%Throughout the experiment, we monitor signal strength quality and handovers on both LTE connections at per-second intervals.

%\begin{table}[!t]
%\centering
%\begin{tabular}{c|ccc}
%Mobility & Goodput (Mbps) & RTT (ms)      & Bytes in Flight \\ \hline
%Stationary   & $72\pm8.6$       & $54\pm2.1$      & $648\pm87$      \\
%Walking  & $58\pm11.7$      & $68\pm11.6$     & $534\pm131$     \\
%Driving  & $43\pm19.4$      & $85\pm12.2$ & $417\pm122$        
%\end{tabular}
%\caption{Results obtained in controlled mobility experiments.}
%	\label{table:control}
%\end{table}

%\subsection{Results} \label{sec:controlResults}

%\begin{figure}[!tb]
%	\centering
%	\includegraphics[width=0.6\linewidth]{Figs/matlab_plots/controlledMobility}
%	\caption{Occurrences of signal strength drops and handovers in five minute segments during controlled experiments.}
%	\label{fig:probChange}
%	%\vskip -3mm
%\end{figure}



%Table \ref{table:control} compares application goodput (in-order bytes
%received per second), mean RTT and mean bytes-in-flight observed in different moving scenarios in our experiments. 
%%
%It can be observed that increasing speeds negatively impacts MPTCP performance in all aspects.

%\smallskip
%\noindent \textbf{Network changes under mobility.} 
%We start by answering the question, \textit{how common are LTE physical link changes in day-to-day mobility?}
%%start by quantifying different physical link changes observed in our experiments. 
%%
%As our data transfers were active throughout the run, we segment our network quality data in \textit{five minute} periods and quantize signal strength drops and handovers observed within each segment.
%% 
%Figure~\ref{fig:probChange} shows the results.
%%number of low to large signal drops, (2-8~dB and $>8$~dB) and handovers observed within data transfer segments. 
%%
%We see that the number of handovers observed by the client during driving far exceeds that while walking.
%%Even though we observed significantly more handovers in driving tests, 
%However, we notice a \textit{"ping-pong"} effect in our walking dataset.
%%
%% our walking frequent handovers in short time intervals in the latter.
%%
%%In several segments, we
%We observe that the client frequently switches between the same set of base stations within a short duration without experiencing signal strength drops. 
%%
%We were unable to find the root cause of this effect but we strongly suspect this behavior due to eNB load balancing algorithms as the effect was prominent in residential areas of the walk.
%%
%Furthermore, our results show that a walking client is likely to experience signal drops of $\approx8$~dBm whereas the intensities of the drops while driving are much higher.
%%while walking a client is more prone to see up to 8db signal strength drops on either LTE connection which is enough to trigger a lower MCS and PHY data rate.
%%
%%As we will show later, this can adversely affect the overall performance of MPTCP.
%%
%%On the other hand, we observed significant signal strength drops coupled with handovers while driving which lead to a notable degradation in MPTCP performance (shown in ).
%
%%Now we investigate the impact of the drop in signal strength and handovers on overall MPTCP performance.
%%\smallskip
%
%\begin{figure}[!t]
%\centering
%\begin{subfigure}{0.235\textwidth}
%\centering
%  \includegraphics[width=\textwidth]{Figs/matlab_plots/line_snrDrop_new}
%  \caption{\label{fig:lineSNR}Signal strength drop}
%\end{subfigure}%
%%\hfill
%\hspace{0.001\textwidth}
%\begin{subfigure}{0.235\textwidth}
%\centering
%  \includegraphics[width=\textwidth]{Figs/matlab_plots/line_Handover_new}
%  \caption{\label{fig:lineHandover}Handover}
%\end{subfigure}
%\caption{Effect of cellular link changes. Throughput graph also shows behavior of TCP flows over each ISP connection.}
%\label{fig:mptcpPhy}
%%\vskip -3mm
%\end{figure}

\smallskip
%\noindent \textbf{Impact of Signal Strength} 
%Figure~\ref{fig:lineSNR} shows MPTCP per-flow performance compared to two regular TCP flows while both connections experience signal drops albeit different intensities.
%%
%It must be noted that Figure~\ref{fig:mptcpPhy} only shows RTT of MPTCP subflows to maintain legibility.
%%
%We observe that while RSSI drop on \ispa signal reduces regular TCP throughput by $\approx33$\%, its impact on MPTCP subflow is far more significant.  
%%We observe that the 4~dB drop in \ispb connection did not impact MPTCP performance as significantly as the 8~dB drop on \ispa signal.
%%
%Our explanation to this behavior is as follows.
%%
%LTE RRM switches to a lower link rate after witnessing drop in signal strength (mapped to a revised MCS) thereby leading to increased buffering at the base station.
%%
%The additional queue delay on the affected path is corroborated by corresponding spikes in RTT and bytes-in-flight (not shown due to space restriction) indicating the presence of bufferbloat.
%%
%%Soon after the drop, the established subflow on \ispa experiences RTT spikes as high as \textit{twice} the mean RTT.
%%
%%We explain this behavior to excessive packet buffering at the base station while the channel switches to a lower bitrate unbeknownst to TCP.
%%
%%This was corroborated by a corresponding increase in bytes-in-flight at the same time (not shown due to space restriction) indicating the presence of bufferbloat.
%%
%Upon noticing the RTT increase, MPTCP \textit{minSRTT} scheduler sends subsequent packets on the other (\ispb) subflow resulting in much lower utilization of \ispa connection, whereas regular TCP continuously buffers packets until the link rate stabilizes.
%%
%We also observe that the time taken by a subflow to recover from queue delays after the signal strength has stabilized far exceeds that of regular TCP. 
%%
%We account this behavior to the design of \textit{minSRTT} scheduler  which restricts packets scheduling on affected path until \ispb subflow experiences higher RTTs. 
%%
%%The presence of  in-network buffers in the core network prevent any packet drops therefore subflow TCP is unable to limit reduce its congestion window size.
%%
%%Although the affected subflow experiences a throughput hit, MPTCP scheduler schedules packets on ISP B subflow which has much lower RTT.
%%
%%This allows MPTCP to overcome intermediate path deterioration while maintaining certain throughput.
%Note that the choice of congestion control does not impact MPTCP performance as no TCP packets were reported dropped or re-transmitted.
%%none of the connections experienced packets drops leading to high window availability on both flows.
%
%%To summarize, our findings show that drop in signal strength impacts MPTCP more significantly than regular TCP.
%%
%%Furthermore, the intensity of the drop has a direct correlation to throughput of the subflow.  
%%shows that out-of-order queue size at the receiver were as large as 1 MB while walking thereby reducing end-application goodput.
  
\smallskip

%handovers on one subflow also adversely affect the performance of another non-affected path.
%
%Considering the large out-of-order queue sizes observed while driving, we suspect throughput reduction to receive buffer stalling experienced by MPTCP.
%
%Packets experiencing very large queue delays due to excessive buffering have potential to remain in receive buffer until they can be delivered in order to the application.
%We attribute this behavior to the large out-of-order queue sizes at the receiver .
%

% experienced during data transfers. 

%\begin{figure}[!tb]
%	\centering
%	\includegraphics[width=0.6\linewidth]{Figs/matlab_plots/outoforderCDF}
%	\caption{Out-of-order queue size distribution with different network conditions.}
%	\label{fig:cdfOFO}
%	%\vskip -3mm
%\end{figure}  

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> mptcp.tex <==
\section{MPTCP at the edge} \label{sec:mptcp_edge}

\subsection{MPTCP in a nutshell} \label{subsec:mptcp_overview}

%\begin{figure}[!tb]
%	\centering
%	\includegraphics[width=0.9\linewidth]{Figs/mptcp_edge}
%	\caption{VM migration between MPTCP-compliant edge servers equipped with multiple interfaces.}
%	\label{fig:model}
%	%\vskip -3mm
%\end{figure}

Unlike regular TCP, MPTCP builds connections over two hosts and not two interfaces.
%
It adds an abstraction control layer atop TCP which is responsible for actively managing packets injected into each connection. 
%
The protocol is composed of three modular control blocks: \textit{path manager}, \textit{scheduler} and \textit{congestion control}.
%
Lets consider a VM migration scenario between two edge servers both equipped with two wireless NICs on both ends.
%
Assuming that both edge servers support MPTCP, the \textit{path manager} is responsible for establishing and managing subflows\footnote{We use the term TCP connection and subflow interchangeably} between the hosts over available NICs.
%
%At time of connection establishment, the path manager at Server A will set MP\_CAPABLE TCP option in its SYN to Server B signaling MPTCP compliance.
%
%Once the inital connection over first NIC has been established, the path manager adds additional subflows over remaining NICs in the same session using ADD\_ADDR TCP option. 
%
%For example, the path manager establishes \textit{four} possible TCP connections, A1-B1, A2-B2, A1-B2, A2-B1 for end-to-end communication (last two not shown). 
%
Once TCP subflows between the machines are established, the \textit{scheduler} injects application packets into each connection while prioritizing network path with lower \textit{sender-perceived} TCP smoothed round-trip time (SRTT).
%
Further, unknowing to underlying TCP, MPTCP adds its end-to-end congestion control and packet sequencing to support out-of-order delivery of packets over heterogeneous paths. 
%
%The underlying TCP connections are unaware of MPTCP's presence and supports individual end-to-end TCP congestion control and sequencing.
%
%its own sequence numbering and \textit{congestion control}, based on same principles of TCP control, to decide the send rate for each subflow.
%
%It must be noted that each TCP subflow also maintains its own congestion window along with MPTCP.
%
%Different congestion control algorithms can be utilized for MPTCP based on underlying requirements but they must ensure that MPTCP always performs better than single-path TCP.
%
%Based on the congestion window size, the \textit{scheduler} decides which subflow should be selected for servicing the packet.
%
%The default scheduler prioritizes the subflow with least TCP round-trip time (RTT) to minimize overall service time.
 
\subsection{Sender vs the Network} \label{subsec:experiment}

\begin{figure}[!tb]
	\centering
	\includegraphics[width=0.78\linewidth]{Figs/retransmission}
	\caption{Default MPTCP operation over two subflows when flow 2 experiences packet errors from $t_1$. MPTCP keeps scheduling new packets to flow 2 resulting in heavy retransmissions over both subflows until RTT of flow 1 exceeds that of flow 2 at $t_2$.}
	\label{fig:plot}
	%\vskip -3mm
\end{figure}

MPTCP architecture is designed to be sender-centric wherein the sender host is primarily responsible for network decisions (packet injection, rate control) based on sender-perceived path information (read SRTT).
%resides  the sender is fully responsible  decisions related to connection establishment, subflow addition, rate control and packet scheduling is taken by the sender.
%
%Majority of these decisions are based on network characteristics, such as RTT, which considers rest-of-the-network (including receiver) as a black box.
%
MPTCP's reliance on sender-focused decisions disables it to timely account for packet delays and losses on the \emph{receiver-side} last mile which, as motivated in Section \ref{sec:intro}, is highly prevalent in today's network.
%We argue that such sender-centric design is fitting in mobile networks where only sender is adjacent to congestion-prone wireless last-hop.
%
%Further, typical applications such as movie streaming, file downloads are not time-critical while being capable of maintaining required QoS despite network delays. 
%sender's last-mile link is wireless and congested whereas the receiver is a datacenter coupled with controlled and managed core network, such protocol design poses no issues as sender is primarily plagued with local network issues.
%
%Furthermore, typical mobile application use-cases such as  movie streaming, file downloads, VoIP etc. are capable of maintaining required QoS despite network delays.
%
%, both underlying network and applications for edge clouds are in stark contrast to that mobile scenarios.
%
%Moreover, typical edge computing use-cases such as VM and container migration are much more latency-stringent where network delays can lead to service disruptions.

To show the impact of MPTCP's behavior, we set up a real edge-to-edge communication experiment discussed in Section \ref{subsec:mptcp_overview}.
%
Both servers are equipped with two 802.11g NICs and support latest default MPTCP v0.94. 
%
Figure \ref{fig:plot} shows per-flow sequence number of packets over time. 
%
We inject path errors on B2 associated with flow 2 starting $t_1$ with 0.2 probability, which triggers increased TCP retransmissions on affected path due to retransmission timeouts (RTO).  
%two edge servers show a graph based on real experimentation about how many RTTs later does the sender realize the issue that one of the path is experiencing problems and how many retransmissions does it take to recover.
%
%Further, MPTCP tries to recover from failures by re-delivering lost packets on the unaffected flow leading to bandwidth wastage (first expanded plot).
%
However, MPTCP keeps injecting new packets on affected flow 2 even after encountering errors, until the delay is reflected in its TCP SRTT (at $t_2$).
%
After $t_2$ all lost packets are retransmitted on unaffected flow 1.
%
%The time difference between when flow 2 experiences losses and when MPCTP limits its usage is due to MPTCP's reliance on TCP exponential weighted average RTT where newer value is only given 20\% consideration.
%      
We found that MPTCP injected 43\% new packets on flow 2, of which 74\% had to be re-transmitted.
%
Such heavy re-transmissions lead to large receive buffers, re-ordering delays and bandwidth wastage. %for overlying applications. 
%[Need to write more about this once figure is attached]

==> receiver-assisted.tex <==
\section{Receiver-assisted MPTCP}

We focus on redesigning MPTCP to incorporate network \emph{reliability} and reduce time delays due to retransmissions and packet reordering in congestion-prone networks. 
%
Receiver-Assisted MPTCP (\textit{RAMPTCP}) is an extension to MPTCP which enables the sender to consider receiver-side last-mile characteristics in its control decisions actively. %
%
We draw \sysname design motivation from TCP congestion control where timely knowledge of receiver's congestion window is pivotal for sender rate control decisions.
%
%Instead of vaguely capturing network and the receiver conditions as RTT, \sysname proposes to make receiver-side network characteristics an active part of sender decisions.
%\sysname design is motivated by TCP congestion control .
%
In experiment above, we observe that the sender continually receives ACKs on either subflow despite packet losses on one flow. 
%unaffected flow 1 within $t_1$ and $t_2$ which could be leveraged to inform sender of losses on interface B2.
%
\sysname facilitates the receiver to report several local last-hop metrics by leveraging reverse-path ACKs to sender. 
%which it can leverage to estimate packet delays at the receiver.
%
%
As \sysname is a work-in-progress, in the following sections we discuss several "possible" design aspects to incorporate receiver characteristics effectively.% changes in MPTCP control block and packet format to enable \sysname.
%However, the sender-centric design of default MPTCP does not leverage any receiver-side information.
 
%can decouple receiver-side delays from RTT for better send decisions.
%
%Unlike single-path TCP connection, MPTCP enables sender to effectively shape the traffic over the network. 
%
%Therefore, knowledge of current network characteristics other than a vague approximation of RTT can enable \sysname to improve network utilization.
%
%
%Being a work-in-progress, we list out several criterion which need to be considered in its protocol design and discuss several open research problems in incorporating receiver network characteristics in \sysname.
%
%(Maybe?) Finally, we show by proof-of-concept evaluation the possible gains if we just consider receiver-side NIC queue sizes for making sender scheduling decisions and discuss what other possible decisions can impact reliability over MPTCP.

%In this section we describe the working on receiver MPTCP.
%%
%Essentially we cover the idea in the following subsections.


\subsection{System design} \label{subsec:design}

\begin{figure}[!tb]
	\centering
	\includegraphics[width=0.87\linewidth]{Figs/ramptcp}
	\caption{\sysname in action.}
	\label{fig:design}
	%\vskip -3mm
\end{figure}

Figure \ref{fig:design} portrays the experiment scenario discussed in Section \ref{subsec:experiment} where receiver-side last hop (B2) is error-prone due to channel interference.
Therefore,  all packets sent on path 2 is dropped at B2's access point.
%%%
%%%Building up on the same scenario discussed in Section \ref{sec:mptcp_edge}, Figure shows the sender edge server (left-side) sending data over two available paths.
%%%
%%%The paths are mapped to two wireless NICs at the receiver edge server (right-side) of which one of the path is error-prone.
%%%
%%%Oblivious to the local path conditions at the receiver, the sender sends a data packet on each path at connection start.
%%%
%The data packet sent by sender on flow 1 (Seq: 1) is successfully delivered to receiver and packet on flow 2 (Seq: 2) is dropped at receiver's access point.
%%
\sysname enables the receiver to report back last-hop metrics such as path loss, channel utilization, SNR, queue length, channel interference, etc. to the sender via modified MPTCP ACK. 
%
This information effectively captures any packet delays/losses at receiver last-hop and is \emph{readily available} in default Linux kernel.  
%%    
The receiver embeds the selected characteristics along with their unique MPTCP \emph{path ID} in all ACKs (for any path) to ensure its delivery.
%%
%The operation of \sysname sender departs from that of regular MPTCP sender which keeps scheduling packets on affected path until its perceived RR exceeds that of the other path. 
%
The sender leverages received path information and augments it with local path characteristics and SRTT to estimate packet delays at sub-network level.
%
Essentially, \sysname breaks down overall SRTT in
%
\begin{align*}
\text{SRTT} = \text{T}_{sender} + \text{T}_{core} + \text{T}_{receiver},
\label{eqn:rtt}
\end{align*}
%
i.e., time delay at sender last-hop, core network and receiver last-hop respectively.
%
To estimate $\text{T}_{sender}$ and $\text{T}_{receiver}$, \sysname can utilize similar principles as sender-side MAC-aware methodologies \cite{crosslayer_infocomm, qaware-ifip} and is thereby able to estimate time delay in core network.
%
By computing per-segment delay for each subflow, \sysname can enforce several control decisions for affected flow quickly, a few of which are listed below.

\noindent\textbf{Scheduler:} limit packet injections, out-of-order injection for heterogeneous delays, packet duplication.

\noindent\textbf{Congestion control:} lower/increase TCP send rate.

\noindent\textbf{Path manager:} boycott subflow usage, utilize subflow using the best combination of last-hop links.
 
 
%By breaking down RTT into its network delay components for each path, \sysname  can limit the utilization of the affected path by explicitly reducing that flow's send rate or boycotting that path from its scheduling decisions until the situation improves.
%
%We must clarify that the control block of \sysname aims to reduce end-to-end packet reordering and retransmission delays, and its end decisions are not limited to that mentioned above.
  
%\subsection{Benefits}
%
%Unlike end-to-end delay estimate based approaches, \sysname optimizes subflow usage by prioritizing reliability over faster packet transmission.
%%
%It aims to reduce packet retransmissions on all subflows thereby increasing effective packet delivery.
%%
%Further, as \sysname is aware of delays at every phase of the network, it also has the capability to deliver MPTCP packets out-of-order from the sender which arrive at the receiver in-order thereby reducing time and buffer spent for re-ordering at the receiver.

\subsection{Preliminary Results}

\begin{figure}[!tb]
	\centering
	\includegraphics[width=0.88\linewidth]{Figs/results}
	\caption{Per-flow throughput comparison between MPTCP and RAMPTCP for topology in Figure \ref{fig:model} when interference on B1 affects flow 1 from 2-5s}
	\label{fig:result}
	%\vskip -3mm
\end{figure}

To evaluate the effectiveness of \sysname, we implement the topology shown in Figure \ref{fig:design} in the ns3 network simulator. 
%
Both source and destination are equipped with two 802.11g NICs associated to their respective APs on orthogonal channels. 
%
The source is aware of receiver channel utilization, SNR and path loss \%. 
%
Figure \ref{fig:result} shows per-flow throughput achieved on both subflows when flow 1 encounters high packet loss due to WiFi interference on the B1 interface from 2-5s. 
%
In its preliminary stage, we design \sysname to simply mark a subflow active/inactive based on \textit{channel interference} and \textit{signal strength threshold}.
%
While MPTCP relies on RTO's to invoke congestion control, \sysname avoids possible packet losses by marking flow 1 "inactive" based on reverse-path information from the destination for the affected time.
%
Overall, \sysname achieves $\approx58\%$ reduction in retransmissions and $\approx19\%$ increase in application goodput.


==> relatedwork.tex <==
\section{Related Work} \label{sec:related}

%Broadly in three sections.

%First is study of TCP in LTE networks. What parameters have people looked at and basic overview of their analysis.
%The development and deployment of LTE led to a vast range of work studying the impact of LTE on networks.
We categorize relevant works into two groups: study and solutions of TCP over LTE and MPTCP in multi-LTE networks.

\smallskip
\noindent \textbf{TCP over LTE.}
%TCP was developed for static wired environment which is different from the dynamic cellular and wireless networks we see today. With the vast deployment of LTE its imperative to study its impact on the TCP performance.
%Merz \textit{et al.}~\cite{merz2014} focused on studying spectral efficiency and resource block utilization among multiple users but do not analyze TCP performance over LTE.
%
Huang \textit{et al.} ~\cite{huang2012,huang2013} analyze the impact of LTE over several parameters such as flow size, time of the day, etc. on TCP. 
%
The authors highlight the underlying problem of the undesirable slow start prevalent in cellular networks. 
%However, they do not take into account behaviour of different congestion control algorithm at high speed. 
Xiao \textit{et al.}~\cite{tcpConcise2014} conduct a measurement study of TCP over LTE in the high-speed rail network. 
%
In~\cite{xu2017}, authors attribute poor TCP performance in high mobility environments to delays in connection establishment, high spurious RTOs, aggressive congestion window reduction, and transmission interruptions.
%
In~\cite{nguyen2014,li2016} the authors study the impact of handovers and increasing distance between user and eNB on TCP throughput.
%
Robert \textit{et al.}~\cite{robert2016} study the behavior of different TCP variants in simulated LTE environments. 
%
%\smallskip
%\noindent \textbf{Improving TCP over cellular.}
%There are few papers that propose new congestion control algorithms designed to improve TCP performance in dynamic cellular networks.
%Remy~\cite{winstein2013tcp} proposes a machine generated congestion control algorithm. %The machine is trained offline and Remy uses the prior knowledge of the network to obtain the desired design goals .
In~\cite{pacifico2009}, the authors propose solutions to avoid high delays during handovers which lead to sub-optimal TCP performance.
%
In~\cite{sivaraman2014}, authors use Remy~\cite{winstein2013tcp} as a design tool to learn the congestion control in unknown network environments.
%
Sprout~\cite{winstein2013} is a congestion control protocol that aims to reduce the TCP delays caused by in-network packet buffering in cellular networks.
%Sprout manages to achieve good throughputs with lower delays.
Zaki \textit{et al.}~\cite{zaki2015} propose Verus which uses RTT gradient to infer congestion for networks. 
%
Verus adapts its sending rate following a delay to bandwidth mapping based on learning during the training.

\smallskip
\noindent \textbf{MPTCP over multiple LTE.}
Authors in~\cite{mptcpmore} study MPTCP over multiple LTE connections but only focus on understanding bandwidth aggregation gains in static environments.
%
Li \textit{et al.}~\cite{li2018} study performance of MPTCP over the cellular network in high-speed rail. 
%
Their observations show that MPTCP performs better than TCP in poorer of the two paths but worse on the better path due to frequent handovers.
%The key takeaway of their work was to show that MPTCP performs better than TCP in poorer of the two paths but worse on the better path due to frequent handovers.
%
In~\cite{zhang2018} authors propose receiver adaptive incremental delay that minimizes out-of-order packets in the heterogeneous multipath cellular transmissions by deploying a Multipath Mobile Router and Aggregation Router.
%
%The need for the addition hardware renders this solution impractical for large scale usage.
%
Sinky \textit{et al.}~\cite{sinky2016} propose a handover-aware cross-layer assisted congestion control algorithm for MPTCP.
%but test it only in simulation.
%
However, the authors test their solution in simulation as it is not feasible in real networks. 

% is a measurement study of the performance of LTE at different speeds (upto 70 mph) in comparison to other mobile networks.

%Next is the solutions proposed for better handling LTE networks (insert Sprout, Adaptive bla bla).

%Third, study of MPTCP in LTE and their basic analysis.,

%Followed by how we are different.
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> uncontrolledExperiments.tex <==
\section{Measurements In-The-Wild} 

%throughput
%We complement our controlled experiments by measuring MPTCP performance in unrestricted setting.
%
%Our data collection over five months covered several transportation modes and speeds, e.g. walking, cars, buses, trains, metro, trams etc.
%

%Next we discuss the results from our experiments and provide explanations to MPTCP behavior under mobility.

%\subsection{How "Multi-Path" is MPTCP?}

%We first focus our analysis on understanding advantages of MPTCP over single TCP flow in cellular mobility.
%
%Our findings from this analysis will act as a reality check for usability of MPTCP as core transport mechanism.
%
%We conduct parallel TCP experiments alongside MPTCP which run same application for each ISP connection.
%
%Further, we classify and compare MPTCP and TCP results obtained for different mobility categories.
% 
%We classify single path TCP data traces collected over each ISP network into same mobility categories as mentioned above and compare it with that of MPTCP.
%
%MPTCP employs default configurations along with CUBIC congestion control and underlying workload is HTTP file download.

%%throughput
%\begin{figure}[!t]
%\centering
%\begin{subfigure}{0.325\linewidth}
%\centering
%  \includegraphics[width=\textwidth]{Figs/matlab_plots/mptcp_tcp_stable_throughput}
%  \caption{\label{fig:mptcp_tcp_through_stable} Static}
%\end{subfigure}%
%\vspace{0.005\textwidth}
%\begin{subfigure}{0.325\linewidth}
%\centering
%  \includegraphics[width=\textwidth]{Figs/matlab_plots/mptcp_tcp_low_throughput}
%  \caption{\label{fig:mptcp_tcp_through_low}Low mobility}
%\end{subfigure}
%\vspace{0.005\textwidth}
%\begin{subfigure}{0.325\linewidth}
%\centering
%  \includegraphics[width=\textwidth]{Figs/matlab_plots/mptcp_tcp_high_throughput}
%  \caption{\label{fig:mptcp_tcp_through_high}High mobility}
%\end{subfigure}
%\caption{MPTCP vs. TCP throughput in different mobility.}
%\label{fig:throughput_mptcp_tcp}
%%\vskip -3mm
%\end{figure}
%
%%rtt
%\begin{figure}[!t]
%\centering
%\begin{subfigure}{0.325\linewidth}
%\centering
%  \includegraphics[width=\textwidth]{Figs/matlab_plots/mptcp_tcp_delay_stable}
%  \caption{\label{fig:mptcp_tcp_delay_stable} Static}
%\end{subfigure}%
%\vspace{0.005\textwidth}
%\begin{subfigure}{0.325\linewidth}
%\centering
%  \includegraphics[width=\textwidth]{Figs/matlab_plots/mptcp_tcp_delay_low}
%  \caption{\label{fig:mptcp_tcp_delay_low}Low mobility}
%\end{subfigure}
%\vspace{0.005\textwidth}
%\begin{subfigure}{0.325\linewidth}
%\centering
%  \includegraphics[width=\textwidth]{Figs/matlab_plots/mptcp_tcp_delay_high}
%  \caption{\label{fig:mptcp_tcp_delay_high}High mobility}
%\end{subfigure}
%\caption{MPTCP vs. TCP queue delays in different mobility.}
%\label{fig:delay_mptcp_tcp}
%%\vskip -3mm
%\end{figure}
%
%%bif
%\begin{figure}[!t]
%\centering
%\begin{subfigure}{0.325\linewidth}
%\centering
%  \includegraphics[width=\textwidth]{Figs/matlab_plots/mptcp_tcp_bif_stable}
%  \caption{\label{fig:mptcp_tcp_bif_stable} Static}
%\end{subfigure}%
%\vspace{0.005\textwidth}
%\begin{subfigure}{0.325\linewidth}
%\centering
%  \includegraphics[width=\textwidth]{Figs/matlab_plots/mptcp_tcp_bif_low}
%  \caption{\label{fig:mptcp_tcp_bif_low}Low mobility}
%\end{subfigure}
%\vspace{0.005\textwidth}
%\begin{subfigure}{0.325\linewidth}
%\centering
%  \includegraphics[width=\textwidth]{Figs/matlab_plots/mptcp_tcp_bif_high}
%  \caption{\label{fig:mptcp_tcp_bif_high}High mobility}
%\end{subfigure}
%\caption{MPTCP vs TCP bytes-in-flight in different mobility.}
%\label{fig:bif_mptcp_tcp}
%%\vskip -3mm
%\end{figure}

%\begin{figure}[!tb]
%	\centering
%	\includegraphics[width=0.45\linewidth]{Figs/matlab_plots/signalDrop_small}
%	\caption{Impact of signal strength drop on normalized RTT.}
%	\label{fig:snrDropRTT}
%	%\vskip -3mm
%\end{figure}
%
%\begin{figure}[!tb]
%	\centering
%	\includegraphics[width=0.45\linewidth]{Figs/matlab_plots/handoverCDF_small}
%	\caption{Distribution of normalized RTT with network changes.}
%	\label{fig:cdfRTT}
%	%\vskip -3mm
%\end{figure}


\subsection{Diving Deep in Network Changes}

To seek the root cause for MPTCPs ineffective bandwidth utilization, we study the impact of network quality changes on each subflow.
%
We calculate \textit{normalized RTT} by normalizing per-packet RTT over initial RTT recorded at connection establishment,
%as this value closely represents the scenario when there were no queue build ups in the network.
%
and further average all normalized RTTs observed within \textit{one second} when a subflow experiences signal strength drop or handover. 
%
This allows us to track the impact of network state change to induced delay.
% 
Our results are shown in Figure~\ref{fig:snrDropRTT}.
%
%As we did not observe any significant affect of 2dB drop on RTT, we exclude those values in the result shown.
We observe that increasing signal drop intensity produces larger RTT spikes where a subflow can experience an increase in RTTs upto \textit{ten} times its static value (500~ms over 50~ms in Table~\ref{table:control}). 
%We observe that increasing intensity of signal drops leads to larger RTT spikes wherein a flow is likely to experience instantaneous RTTs upto \textit{ten} times its value observed in static condition (500ms over 50ms shown in Table~\ref{table:control}). 
%
As discussed in Section~\ref{sec:controlled}, such large instantaneous delay differences between LTE connections fuels ineffective MPTCP scheduling triggering a domino effect of performance degradation due to receive buffer blocking and packet reordering.

As large RSSI drops are often accompanied by a subsequent handover, we isolate the aftermath of both network changes.
%
We remove all observed network states from our dataset where a drop in signal was immediately followed by a handover as resulting effect on performance can be induced by either of the two. 
%
The plot showing distribution of normalized RTTs observed over isolated signal drops and handovers is shown Figure~\ref{fig:cdfRTT}.
%The result explains the extent of underlying queue build-ups on TCP performance and explains the results we observed in Section \ref{sec:controlResults}
%
%We observe that TCP observes significant RTT spikes with increase in signal strength drop reaching as high as \textit{15 times} mean RTT in static condition.
%
%Figure  compares CDF of normalized RTTs for signal strength drops and handovers.
%
%Our results corroborate previous studies which have also observed significant TCP RTTs due to large in-network queue delays.
%
It can be inferred that \textit{handovers are more probable cause of performance disruptions in MPTCP than signal drops} as larger RTT spikes can lead to larger OFO queue sizes and many-second outages.
%
Furthermore, in high mobility where all underlying subflows experience handovers frequently and at different times, there is a strong need for an effective scheduling policy which can remove packets from a congested flow undergoing handover to other available paths.
%The problem of extreme RTT spikes due to handovers is further aggravated by unpredictability of underlying cellular network and reluctance of cellular operators to dropping packets in large-queues.
%
%Furthermore, rather than taking union of individual subflow performances under mobility, default MPTCP acts as an intersection.
%
%This behavior can be largely attributed to ineffectiveness of the default scheduler and its reliance on RTT as core decision metric. 




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

